Spinor Bose-Einstein condensates

An overview on the physics of spinor and dipolar Bose-Einstein condensates (BECs) is given. Mean-field ground states, Bogoliubov spectra, and many-body ground and excited states of spinor BECs are discussed. Properties of spin-polarized dipolar BECs and those of spinor-dipolar BECs are reviewed. Some of the unique features of the vortices in spinor BECs such as fractional vortices and non-Abelian vortices are delineated. The symmetry of the order parameter is classified using group theory, and various topological excitations are investigated based on homotopy theory. Some of the more recent developments in a spinor BEC are discussed.

==> super.tex <==
\section{Superflow, Spin current, and Berry's phase}

\subsection{Mass and spin supercurrent}
In this section, we consider the spatial variation of the order parameters, which
can generate mass and spin supercurrents.

\subsection{spin-1 ferromagnetic phase}
One representation for the spin-1 ferromagnetic order parameter is given by ${\bm \zeta}=(1,0,0)^T$.
Since the polarization direction is arbitrary at zero magnetic field,
a general form of the ferromagnetic order parameter is obtained by
spin rotation $U(\alpha,\beta,\gamma) \equiv e^{-iS_z \alpha} e^{-iS_y \beta} e^{-iS_z \gamma}$ together with a gauge transformation $e^{i\phi}$,
where $\alpha, \beta$ and $\gamma$ are Euler angles.
For a spin-1 system, $U(\alpha,\beta,\gamma)$ is given by
\begin{align}
U(\alpha,\beta,\gamma)
&= \begin{pmatrix}
e^{-i(\alpha+\gamma)} \cos^2 \frac{\beta}{2} \ & \;
-\frac{e^{-i\alpha}}{\sqrt{2}} \sin \beta \ & \; e^{-i (\alpha-\gamma)}
\sin^2 \frac{\beta}{2} \\[2mm]
\frac{e^{-i\gamma}}{\sqrt{2}} \sin \beta \ & \; \cos \beta \ & \;
-\frac{e^{i\gamma}}{\sqrt{2}} \sin \beta \\[2mm]
e^{i(\alpha-\gamma)} \sin^2 \frac{\beta}{2} \ & \;
\frac{e^{i\alpha}}{\sqrt{2}} \sin \beta \ & \; e^{i(\alpha+\gamma)}
\cos^2 \frac{\beta}{2}
\end{pmatrix}.
\label{eqSCB87}
\end{align}
The general order parameter of a spin-1 ferromagnetic state is given by
\begin{align}
{\bm \zeta}_{\rm F} = e^{i\phi}U(\alpha,\beta,\gamma)\begin{pmatrix} 1\\0\\0\end{pmatrix}
= e^{i(\phi-\gamma)}
\begin{pmatrix}
e^{-i\alpha}  \cos^2 \frac{\beta}{2} \\[1mm]
\frac{1}{\sqrt{2}} \sin \beta \\[1mm]
e^{i\alpha} \sin^2 \frac{\beta}{2}
\end{pmatrix}.
\label{eqSCB88}
\end{align}


\begin{align}
{\bm v}^{\rm (mass)} &= \frac{\hbar}{M}\left[\nabla(\phi-\gamma)-(\nabla \alpha)\cos\beta\right]\\
{\bm v}^{\rm (spin)}_\mu &= f_{\mu} {\bm v}^{\rm (mass)} -\frac{\hbar}{2M} \epsilon_{\mu\nu\lambda}f_\nu\nabla f_\lambda 
\end{align}


Symmetry of the system locally breaks
so that $\alpha, \beta, \gamma$ and $\phi$ depends on space.


The linear combination $(\phi-\gamma)$ in Eq.~\eqref{eqSCB88} reflects the continuous spin-gauge symmetry, i.e., the equivalence between phase change and spin rotation.
The physically different configurations of ${\bm \psi}_{\rm F}$ are given by the full range of the Euler angles ($\alpha,\beta$ and $\gamma-\phi$).
Consequently, the order-parameter manifold is $R_{\rm F}={\rm SO}(3)_{\bm S,\phi}$.

The general order parameter of a spin-1 polar state is given by
\begin{align}
{\bm \psi}_{\rm P} = e^{i\phi}U(\alpha,\beta,\gamma)\sqrt{\rho}\begin{pmatrix} 0\\1\\0\end{pmatrix}
= \sqrt{\rho}\,e^{i\phi}
\begin{pmatrix}
-\frac{e^{-i\alpha}}{\sqrt{2}} \sin\beta \\
\cos\beta \\
\frac{e^{i\alpha}}{\sqrt{2}} \sin\beta
\end{pmatrix}.
\label{eqSCB95}
\end{align}
Here, ${\bm \psi}_{\rm P}$ is independent of $\gamma$ and reflects the ${\rm U}(1)_{S_z}$ symmetry.
The order parameter is expressed with $\phi$ and the direction of the spin quantization axis ${\bm d}=(\cos\alpha \sin\beta, \sin\alpha\sin\beta, \cos\beta)$.
The manifold for $\bm d$ constitutes a unit sphere called 2-sphere $S^2$.
Since ${\bm \psi}_{\rm P}$ is invariant under the simultaneous transformations  $(\phi,{\bm d})\to (\phi+\pi,-{\bm d})$, a direct product of $S^2$ for $\bm d$ and U(1) for $\phi$ covers the order-parameter manifold twice. 
Therefore, $R_{\rm P} = (S^2_{\bm S} \times {\rm U}(1)_\phi)/({\mathbb Z}_2)_{\bm S,\phi}$.
The order-parameter manifolds for various phases of spin-2 BECs are summarized in Table.~\ref{tb:coset_space}.

\begin{table}
\begin{tabular}{ll|lll}
 \ spin-1        & $R$ &\  spin-2 & $R$\\ \hline
 \ ferromagnetic\  & ${\rm SO}(3)_{\bm S,\phi}$\ \ \ \  
&\ ferromagnetic\  & ${\rm SO}(3)_{\bm S,\phi}$\\[1mm]
 \ polar         & $\frac{S^2_{S}\times {\rm U}(1)_\phi}{({\mathbb Z}_2)_{\bm S,\phi}}$\  
 & \ uniaxial nematic     & $\frac{S^2_{\bm S} \times U(1)_\phi}{({\mathbb Z}_2)_{\bm S}}$ \\[2mm]
&& \ biaxial nematic I  & $\frac{{\rm SO}(3)_{\bm S} \times U(1)_\phi}{({\mathbb Z}_4)_{\bm S,\phi}}$ \\[2mm]
&& \ cyclic      & $\frac{{\rm SO}(3)_{\bm S} \times U(1)_\phi}{T_{\bm S,\phi}}$\ \ \ \ \\
\end{tabular}
\caption{Coset space for various phases of spin-1 and spin-2 spinor BECs}
\label{tb:coset_space}
\end{table}

